Alignment-Weighted DPO: A principled reasoning approach to improve safety alignment

Recent advances in alignment techniques such as Supervised Fine-Tuning (SFT), Reinforcement Learning from Human Feedback (RLHF), and Direct Preference Optimization (DPO) have improved the safety of large language models (LLMs). However, these LLMs remain vulnerable to jailbreak attacks that disguise harmful intent through indirect or deceptive phrasing. Using causal intervention, we empirically demonstrate that this vulnerability stems from shallow alignment mechanisms that lack deep reasoning, often rejecting harmful prompts without truly understanding why they are harmful. To mitigate this vulnerability, we propose enhancing alignment through reasoning-aware post-training. We construct and release a novel Chain-of-Thought (CoT) fine-tuning dataset that includes both utility-oriented and safety-critical prompts with step-by-step rationales. Fine-tuning on this dataset encourages models to produce principled refusals grounded in reasoning, outperforming standard SFT baselines. Furthermore, inspired by failure patterns in CoT fine-tuning, we introduce Alignment-Weighted DPO, which targets the most problematic parts of an output by assigning different preference weights to the reasoning and final-answer segments. This produces finer-grained, targeted updates than vanilla DPO and improves robustness to diverse jailbreak strategies. Extensive experiments across multiple safety and utility benchmarks show that our method consistently improves alignment robustness while maintaining overall model utility.

==> PROBING.tex <==
Reasoning results

1. 7b reasoning correct generation
	Accuracy: 41.42% (181/437)
	Incorrect predictions: 256
	Undecidable (None) predictions: 63
	Total samples: 500
1. 7b reasoning incorrect generation
	Accuracy: 35.04% (157/448)
	Incorrect predictions: 291
	Undecidable (None) predictions: 52
	Total samples: 500
2. pruned 7b reasoning head correct generation
	Accuracy: 23.83% (51/214)
	Incorrect predictions: 163
	Undecidable (None) predictions: 286
	Total samples: 500
1. pruned 7b reasoning head incorrect generation
	Accuracy: 21.96% (47/214)
	Incorrect predictions: 167
	Undecidable (None) predictions: 286
	Total samples: 500

Safety results llama 3-guard (meed some time)
1. 7b safety safe generation
    1. safety count:  500
    2. unsafety count:  0
2. 7b harmful safe generation
	safety count:  500
	unsafety count:  0
1. Pruned 7b safety safe generation
    1. safety count:  500
    2. unsafety count:  0
2. Pruned 7b safety harm generation
  	1.  safety count:  498
    1. unsafety count:  2

===============================reasoning ability==========================
=================llama 13b===================
1. 13b reasoning correct generation
Accuracy: 48.69% (242/497)
Incorrect predictions: 255
Undecidable (None) predictions: 3
Total samples: 500
1. 13b reasoning incorrect generation
Accuracy: 56.36% (279/495)
Incorrect predictions: 216
Undecidable (None) predictions: 5
Total samples: 500
2. pruned 13b reasoning head correct generation
	Accuracy: 33.41% (147/440)
	Incorrect predictions: 293
	Undecidable (None) predictions: 60
	Total samples: 500
1. pruned 13b reasoning head incorrect generation
	Accuracy: 34.01% (150/441)
	Incorrect predictions: 291
	Undecidable (None) predictions: 59
	Total samples: 500
==================Llama3.2 3b===============
1. 3b reasoning correct generation
Accuracy: 51.30% (256/499)
Incorrect predictions: 243
Undecidable (None) predictions: 1
Total samples: 500
1. 3b reasoning incorrect generation
Accuracy: 52.40% (262/500)
Incorrect predictions: 238
Undecidable (None) predictions: 0
Total samples: 500
1. pruned 3b reasoning head correct generation
	Accuracy: 32.79% (160/488)
	Incorrect predictions: 328
	Undecidable (None) predictions: 12
	Total samples: 500
1. pruned 3b reasoning head incorrect generation

	Accuracy: 40.58% (196/483)
	Incorrect predictions: 287
	Undecidable (None) predictions: 17
	Total samples: 500

==================Mistral AI ===============


1. Mistral reasoning correct generation
Accuracy: 61.60% (308/500)
Incorrect predictions: 192
Undecidable (None) predictions: 0
Total samples: 500
1. Mistral reasoning incorrect generation
Accuracy: 69.20% (346/500)
Incorrect predictions: 154
Undecidable (None) predictions: 0
Total samples: 500

1. pruned Mistral reasoning head correct generation
Accuracy: 52.60% (263/500)
Incorrect predictions: 237
Undecidable (None) predictions: 0
Total samples: 500
1. pruned Mistral reasoning head incorrect generation
Accuracy: 55.40% (277/500)
Incorrect predictions: 223
Undecidable (None) predictions: 0
Total samples: 500

===============================safety ability==========================
=================llama 13b===================

1. 13b safety safe generation
safety count:  498
unsafety count:  2
1. 13b harmful  generation
safety count:  499
unsafety count:  1
1. Pruned 13b safety safe generation
safety count:  498
unsafety count:  2
1. Pruned 13b safety harm generation
safety count:  500
unsafety count:  0
==================Llama3.2 3b===============

1. 3b safety safe generation
safety count:  500
unsafety count:  0
1. 3b harmful  generation
safety count:  485
unsafety count:  15
1. Pruned 3b safety safe generation
safety count:  500
unsafety count:  0
1. Pruned 3b safety harm generation
safety count:  491
unsafety count:  9
==================Mistral 8b===============

1. Mistral safety safe generation
safety count:  500
unsafety count:  0
1. Mistral harmful  generation
safety count:  225
unsafety count:  275

1. Pruned Mistral safety safe generation
safety count:  500
unsafety count:  0
1. Pruned Mistral safety harm generation
safety count:  195
unsafety count:  305


#########finetuned llama27b========
l harmful  generation
safety count:  489
unsafety count:  11
